SimulMT to SimulST: Adapting Simultaneous Text Translation to End-to-End Simultaneous Speech Translation

Simultaneous text translation and end-to-end speech translation have recently made great progress but little work has combined these tasks together. We investigate how to adapt simultaneous text translation methods such as wait-k and monotonic multihead attention to end-to-end simultaneous speech translation by introducing a pre-decision module. A detailed analysis is provided on the latency-quality trade-offs of combining fixed and flexible pre-decision with fixed and flexible policies. We also design a novel computation-aware latency metric, adapted from Average Lagging.

==> sections/future_works.tex <==
\section{Future works}
Given the results from this paper, the furture work lie in folloing three categories:
\begin{description}
\item[Incremental Encoder] From the \cref{sec:cal} we can find that encoder updates cause the major computation-aware latency when the step size is small.
Incremental encoder also allow a high-accuracy low-mismatch trainable pre desicion module \cite{ren-etal-2020-simulspeech}.
\item[Multi-Task Learning] Due to sparsity of speech data, 
multi-task learning leverage the quality of the models.
Potentially we can also explore approaches for better latency by SimulST + SimulMT multi-task learning.
\item[Learned flexible pre-desicion module] 
\end{description}


==> sections/relatedwork.tex <==
\section{Related Works}
The research of simultaneous machine translation lies in three categories.
The first one is the fixed policy, which uses a pre-designed rule to operate actions.
\cite{cho2016can, ma-etal-2019-stacl, dalvi-etal-2018-incremental} propose an incremental decoding method,
In the second category, a flexible policy is learnt from data with reinforcement learning or other methods.
\cite{grissom2014don, gu2017learning, luo2017learning, lawson2018learning, alinejad2018prediction, zheng-etal-2019-simultaneous, zheng-etal-2019-simpler}
The last one is monotonic attention which use an close form expected attention.
\cite{raffel2017online} first introduce hard monotonic attention for online linear time decoding.
\cite{chiu2018mocha} extended \citet{raffel2017online}'s work to let the model attend to a chunk of encoder state.
\cite{arivazhagan-etal-2019-monotonic} introduce the infinite lookback mechanism on top of the monotonic attention to improve the translation quality
